Impacts of packed bed polydispersity and deformation on fine particle transport

Static granular packings play a central role in numerous industrial applications and natural settings. In these situations, fluid or fine particle flow through a bed of static particles is heavily influenced by the narrowest passage connecting the pores of the packing, commonly referred to as pore throats or constrictions. Existing studies predominantly assume monodisperse rigid particles, but this is an oversimplification of the problem. In this work, we illustrate the connection between pore throat size, polydispersity, and particle deformation. Simple analytical expressions are provided to link these properties of the packing, followed by examples from Discrete Element Method (DEM) simulations of fine particle percolation demonstrating the impact of polydispersity and particle deformation. Our intent is to emphasize the substantial impact of polydispersity and particle deformation on constriction size, underscoring the importance of accounting for these effects in particle transport in granular packings.

==> figs/song/chapter4.tex <==
\chapter{Geometric constraints for fine particle percolation in static beds of size-polydisperse spherical particles}
\label{chap:porewidth}


 \begin{center}
SUMMARY
 \end{center}


The packing of spherical particles has long been recognized as a classic model for various types of porous media, such as rocks and soils in a wide range of geological settings. By understanding the fundamental physical properties of static packings, including packing density, permeability, and pore size distribution, insights can be gained for understanding various transport phenomena. However, compared to the extensive study on the packing of identical spheres, packing of particles having different sizes has received relatively less attention in research. Nevertheless, such packings are more representative of the actual static arrangements of particles found in nature and industry. Here, we investigate the structure of static beds comprised of spherical particles with variations in size. Building upon previous research that has shown the influence of size dispersity on packing density~\cite{farr2009close,baranau2014random}, we demonstrate, both theoretically and using discrete element method simulations, that the pore-throat size distribution and its lower bound (which determines the free-sifting threshold) are affected by the width of the bed particle size distribution. This, consequently, leaves a notable impact on the percolation behavior of same fine particles, transitioning from not being trapped in size-monodisperse packings to being trapped within size-polydisperse packings. %These findings have potentials to improve the performance of packed beds in various practical industrial appliances, such as filtration.

The material in this chapter will be incorporated into a manuscript by D. R. Vyas, S. Gao, J. M. Ottino, P. B. Umbanhowar, and R. M. Lueptow that is currently in preparation. The research described in this chapter is entirely my own, though D. R. Vyas working on a related parallel study of the effects of pressure and subsequent particle deformation on the static bed structure and percolation of fine particles.


\section{Introduction}

The packing of particles holds significant relevance across various fields, including fluid and particle flow in porous media for filtration, soil mechanics, sedimentation, and other geological phenomena. A comprehensive understanding of the fundamental physical properties of static packings, including packing density, permeability, and pore size distribution, provides valuable insights into these fields. 

%Using an appropriate mapping method~\cite{farr2009close}, the analysis of packing density and interstitial volume within complex three-dimensional packed beds can be effectively simplified to the packing of two-dimensional circles, which is more amenable to analyze and model. 
The geometry of circles in contact with each other, which provides a geometric basis for this study, has a rich historical background, with its origins dating back to ancient Greece. Apollonius of Perga first extensively studied this problem, and his work on the ``circles of Apollonius'' covers a series of problems related to circle configurations. One famous problem in Euclidean plane geometry, commonly referred to as the ``problem of Apollonius'', is constructing a circle that is tangent to three given circles within a plane. The solution includes a total of eight circles, some of which enclose one or more of the given circles. Of particular interest in our study is one specific solution where the constructed circle does not enclose any of the given circles. This circle defines the open space between the given circles, which provides insights into various practical applications. One such application is the percolation of fine spherical particles within a static bed composed of larger spherical particles, where fine particles fall through the interstices between the larger particles, driven by gravity. This phenomenon is also known as free sifting (or spontaneous percolation).

A key aspect in comprehending free sifting is determining the particle size ratio threshold (or the free-sifting threshold) that allows fine particles to pass freely through the void spaces between static larger particles. The ``problem of Apollonius" plays a significant role in identifying this threshold by aiding in the characterization of the ``pore throat" formed by the bed particles~\cite{gao2023percolation}. The pore throat formed by larger bed particles represents the smallest passage through which fine particles can percolate. The narrowest constraint, i.e., the smallest pore throat, within a static bed formed by identical bed particles occurs when the three bed particles are tangent to each other and form a planar triangle. The size ratio of the bed particle diameter to the diameter of the largest fine that can pass through such formed pore throat is $R_t = d/d_p = \sqrt{3}/(2-\sqrt{3})=6.464$, where $d$ and $d_p$ are the bed particle and pore throat diameter, respectively. This size ratio is called the geometrical trapping threshold~\cite{kerimov2018mechanical}. Numerical and experimental studies conducted after the pioneering work of Dodds~\citep{dodds1980porosity} show that the analogous size ratio for a static randomly packed large particle bed is about 6.67, which is slightly larger than $R_t$ due to the occasional formation of jammed arches of fine particles between large particles~\cite{kerimov2018mechanical}. It is important to note that other factors such as electrostatic forces, adhesion forces, and particle shape all have an impact on the value of $R_t$ required for particle percolation and trapping in practical applications.

In this work, we consider the effects of the size variation of the bed particles on the free-sifting threshold that have come about as a result of our studies on some practical aspects of the fine particle percolation in static beds~\cite{gao2023percolation} and sheared beds (Chapter~\ref{chap:sheared}). This problem, related to the void spaces between packings of spherical particles, is purely geometric in nature but appears to not have been previously addressed in the literature, as best we can tell.  Of course, this is surprising, given that the history of the geometry of circle packings goes back to ancient times. 

In discrete element method (DEM) simulations, it is typically necessary to vary the size of the bed particles to avoid an inadvertent crystal-like packing when a random packing is preferred~\cite{staron2014segregation}. The variation in particle size necessary to avoid crystal-like packing is usually relatively small, i.e., the bed particle size is typically varied by about $\pm 10\%$ around its mean value. Despite this seemingly small variation, it can have a significant impact on the size of pore throats defined by groups of three neighboring bed particles within the packed bed. To account for the effects of bed particle size distribution, our study begins by examining the pore-throat size from a purely geometric perspective. This geometric analysis allows us to understand the relationship between bed particle size variation and changes in the size of pore throats. Then we explore the practical implications on fine particle percolation in static beds, using DEM simulations. 

Although the motivation for this paper and the examples included herein are based on fine particle percolation through a randomly packed bed of large particles, the issue of pore throat size dependence on the the particle size distribution should is relevant in a wide range of situations.  Examples include the flow of a fluid through a bed of slightly deformable particles, the particle trapping efficiency of a bed of particles used for filtration, and the flow of percolating particles through a geologic formation for oil or gas recovery.  In all these cases and many more, the geometry of spherical particle packing, whether related to the actual geometry of the situation that is being considered or related to idealized models for the particular situation like DEM simulations, plays a significant role in the analysis, and the effects of particle overlap/deformation and size variation need to be taken into proper account.


%This problem has many applications. For instance, fine particles are ubiquitous in industrial solids handling processes, which can lead to degraded product quality, fouled equipment, and safety hazards such as dust explosions~\cite{amyotte2010dust,davies1949inhalation}. Another application is geophysical flows where fine particles can act as bearing balls in long-runout landslides when they percolate to the bottom of the flow during the early phase of the landslide, thereby increasing the mobility of the overlying bed of particles during the later phase of the landslide~\cite{phillips2006enhanced,linares2007increased}. Fine sediments also play important role in the surface water ecosystems. The infiltration of sand or clay particles behave differently in the gravel riverbed. Depends on size differences and flow rate, fine sediments may form a sand seal near the top of the bed or percolate and deposit at the bottom~\cite{dubuis2023clogging}.




\section{Analytical solution of the smallest pore throat}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{ch_polyPSD_figures/Figure1.pdf}
    \caption{Free-sifting threshold vs. bed particle size distribution half-width, $w$, for four extreme situations. C1: three smallest particles touch (black solid); C2: three largest particles touch (magenta dashed); C3: two largest and one smallest particles touch (blue dotted); C4: two smallest and one largest particles touch (red dash-dotted). }
    \label{fig:chporefig1}
\end{figure}


When the particles in a static bed are size-polydisperse, i.e., they exhibit size variation, the resulting pore-throat size distribution formed within the static packing becomes a function of the bed particle size distribution. In particular, the size of the smallest pore throat is crucial because it determines the narrowest passageway through the packed bed, or, equivalently, the largest fine particle that can pass through the bed without being trapped. For a static bed formed by particles with a given size distribution, it is reasonable to consider that the smallest pore throat is formed by three touching particles with extreme sizes, either the smallest or the largest bed particles. When the width of the bed particles size distribution is $2w$, bed particle diameter $d$ ranges from $(1-w)d_0$ to $(1+w)d_0$, where $d_0$ is the bed particle diameter corresponding to the midpoint of the particle size distribution. By enumerating the possible combinations of particles with extreme sizes, we can identify four possible scenarios: three smallest particles (C1), three largest particles (C2), one smallest and two largest particles (C3), or one largest and two smallest particles (C4), see Fig.~\ref{fig:chporefig1}. For each scenario, three particles are assumed to be tangent in the same plane. In the two-dimensional circle packing (which is equivalent to the three-dimensional sphere packing), the pore throat is the largest circle fitting to the center opening formed by three touching bed particles. An analytical solution for the pore throat diameter, $d_p$, for these four scenarios can be found as a function of particle size distribution half-width, $w$. Consequently, the effective free-sifting threshold is defined as $R_t=d_0/d_p$. For comparison, the free-sifting threshold formed by identical bed particles (diameter $d_0$) is the well-known value, $R_{t0}=6.464$. 

Such critical size ratio for the C1 case (three smallest particles touch) can be found by first noting that $(1-w)d_0=6.464d_p$, which can be rewritten as
\begin{equation}
R_t=R_{t0}/(1-w).
\label{eq:chporeeq1}
\end{equation}
$R_t$ for the C1 case increases as $w$ increases, which is shown as the black solid curve shown in Fig.~\ref{fig:chporefig1}. This is reasonable as the increase of $w$ leads to the reduction of the diameter of the smallest bed particles, which necessarily form a smaller pore throat, leading to a larger $R_t$ (equivalent to a smaller fine particle being able to fit through the pore throats of the particle bed).

For comparison, the critical size ratio for the C2 case (three largest particles touch), for which $(1+w)d_0=6.464d_p$, is
\begin{equation}
R_t=R_{t0}/(1+w).
\end{equation}
$R_t$ for the C2 case decreases as $w$ increases, see the magenta dashed curve shown in Fig.~\ref{fig:chporefig1}. Again, this is reasonable in that larger largest bed particles result in a large pore throat.

For the C3 condition, we first solve a set of three equations to identify the pore throat radius $r_p$
\begin{equation}
(x_p-x_i)^2+(y_p-y_i)^2=(r_p+r_i)^2,
\end{equation}
where $i=1,2,3$ corresponds to a touching triad of one smallest and two largest bed circles, see Fig.~\ref{fig:chporefig1}. $x_i$ and $y_i$ are the positions of the center of circle $i$, while $r_i$ is the radius of circle $i$. Then the pore throat diameter is obtained using $d_p=2r_p$ and the analytical solution for $R_t=d_0/d_p$ can be written as
\begin{equation}
R_t=\frac{2w/(1-w)+\sqrt{(3+w)/(1-w)}}{2-\sqrt{(3+w)(1-w)}},
\end{equation} 

Similarly, we get $R_t$ as a function of $w$ for the C4 case, expressed as
\begin{equation}
R_t=\frac{-2w/(1+w)+\sqrt{(3-w)/(1+w)}}{2-\sqrt{(3-w)(1+w)}}.
\end{equation}
They are plotted as the red dot-dashed curve and the blue dotted curve in Fig.~\ref{fig:chporefig1}. These two cases lie between the cases for equal size bed particles (C1 and C2).

When the bed particle size distribution half-width, $w$, is zero, corresponding to the monodisperse limit, all bed particles are identical. Thus, $R_t=R_{t0}$ for all four cases at $w=0$. As $w$ increases, the behaviors of  $R_t$ for different cases show different trends. For example, in the C1 case, $R_t$  increases monotonically as $w$ increases. This indicates that a wider bed particle size distribution results in a larger free-sifting threshold, such that a smaller fine particle would be needed to pass through the static bed. On the other hand, in the C4 case,  $R_t$ exhibits a decreasing trend as $w$ increases. However, considering all cases, as $w$ increases, the smallest pore throat is consistently formed by the C1 case. This means that the configuration of three smallest particles in direct contact is the limiting case that results in the smallest available passage within the packed bed, or largest value for $R_t$, regardless of the extent of particle size variation. Consequently, the black curve in Fig.~\ref{fig:chporefig1} represents the lower bound of the pore-throat size distribution within the static bed formed by size-polydisperse bed particles. More specifically, the effective free-sifting thresholds are $R_t=6.464$, 7.182, 8.080, 9.234, 10.774, and 12.928 for $w=$ 0, 0.1, 0.2, 0.3, 0.4, and 0.5, respectively. 

Thus, a slight increase of the bed particle size distribution width can completely change the percolation behavior of a fine particle (with a fixed size) in the static bed from the passing to the trapping regime, as defined previously~\cite{gao2023percolation}. For example, if the large to fine particle size ratio is $R=7$, a fine particle (diameter $d_f=d_0/7$) is never trapped in a static bed formed by monodisperse larger particles (diameter $d_0$)~\cite{gao2023percolation}. However, when the bed particles have a size distribution half-width of $w=0.1$, it’s possible for the same fine particle to be trapped in the static bed, since the effective critical size ratio is 7.182 now. To further consider this effect, we perform several DEM simulations.

\section{Simulation setup}


In the DEM simulations, we first generate bed particles with identical particle diameters, which in this case is set to $d_0=5$ mm. These particles are arranged on a simple cubic lattice within a rectangular domain. To ensure that bed particles do not overlap with each other after the size variation is applied, the unit cell size for the simple cubic lattice is $1.5d_0$. Periodic walls are prescribed in the $x$ and $y$ directions to eliminate the wall effects, which would lead to the phenomenon that void spaces between particles and an impermeable wall are larger than the spaces between particles~\cite{lee2007micaceous,suzuki2008study}. The length and width of the domain are both $20d_0$. Then the diameter of each bed particle is randomly selected between $(1-w)d_0$ to $(1+w)d_0$, considering cases for $w$ in increments of 0.1 from 0 to 0.5. To maximize the occurrence of three touching smallest bed particles, which determines the lower bound of the pore-throat size distribution, the bed particle diameter is set following a volume-based uniform distribution. By using this distribution, the number of the smallest bed particles is significantly larger than the number of the largest bed particles, although the relative number depends on $w$. To achieve this numerically, size-polydisperse bed particle size distributions actually consist of multiple discrete particle sizes that are uniformly distributed across the desired range of the size distribution. To generate smooth particle size distributions, the diameter increment for the discrete particle diameters is set to 0.05 mm. For example, there are 21 different diameters ranging from 4.5 mm to 5.5 mm for $w=0.1$, while 101 different diameters ranging from 2.5 mm to 7.5 mm are used for $w=0.5$. The total volume (or mass since particle density is fixed as 2500\,kg\,m$^{-3}$) of the particles for each diameter is identical. Consequently, the number of bed particles for each particle diameter is different, decreasing as species size increases. For the case with the largest diameter particles ($w=0.5$), there are only 0.87\% bed particles having a size of 7.5 mm but 19.89\% having a size of 2.5 mm. All other cases have a larger number of the largest particles and a smaller number of the smallest particles.

After the size variation is applied, bed particles are released from their initial positions on the cubic lattice and settle down in the periodic box under gravity $g=9.81$ m\,s$^{-2}$ (in the negative $z$-direction). The bed particles are frozen in place, retaining the periodic sidewalls, after their positions have remained unchanged for some time (typically less than 1 s). Exactly 15\,000 bed particles fill the box to form the static bed with bed height ranging from about $25d_0$ to $30d_0$. Due to the constant number of bed particles, static packing of monodisperse particles has the largest total volume (or height), and the total volume of bed particles decreases as the size distribution half-width $w$ increases because of the increasing fraction of smaller bed particles. Similar to the bed height being sensitive to $w$, the packing density also increases from about 0.624 for $w=0$ to 0.655 for $w=0.5$ because smaller bed particles more easily fill the spaces between the larger bed particles. This phenomenon is consistent with the much more pronounced effect for the packing of size-bidisperse particle mixtures~\cite{petit2020additional}. In the bidisperse case, when the large-to-small particle size ratio exceeds five, the packing density can approach 0.85. For this reason and to avoid the free sifting of bed particles themselves, we use $w\leq0.5$, where an overall homogeneous packing can be achieved. 

Single small particles, with identical diameter $d_f$, are added above the free surface at random locations within a height difference less than $2d_0$ at zero initial velocity, and then free fall under gravity. Similar to our previous work, we use single small particles, i.e., small particles do not interact with each other (although they interact with bed particles), to avoid the situation where multiple small particles jam pore throat~\cite{gao2023percolation}. The number of fine particles is 5\,000 in order to provide adequate statistics in one simulation. For the DEM simulation, we use the Hertz contact model with a Young's modulus of $5\times10^7$\,Pa, a Poisson's ratio of 0.4, a coefficient of restitution of 0.8, and a friction coefficient of 0.5. The simulation time step is $5\times10^{-6}$\,s to assure numerical stability, especially for large size ratios. 




\section{Results}

\subsection{Single fine particle percolation in size-polydisperse static beds}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{ch_polyPSD_figures/Figure2.pdf}
    \caption{Fine particle percolation in static beds consisting of particles with different particle size distribution half-widths (a) $w=0$ (monodisperse), (b) $w=0.2$, and (c)  $w=0.3$. Dashed lines are the periodic boundaries for the static beds. Solid lines are the bottom and the free surface (center of the highest bed particle). Red dots show the position of 5\,000 fine particles at $t=1.5$ s. Black solid curves are the number spatial distribution of fine particles as a function of height in the bed.}
    \label{fig:chporefig2}
\end{figure}


To demonstrate the effect of the width of the bed particle size distribution on fine particle percolation, we consider various particle size ratios, above and below $R_t$, in static beds with different $w$, shown in Fig.~\ref{fig:chporefig2}. All snapshots are taken 1.5 s after fine particles are added at the top of the static bed. From Figs.~\ref{fig:chporefig2}(a) to (c), it is evident that the height of the free surface (shown by the top blue horizontal solid line) decreases as $w$ increases, as previously explained. As shown in Fig.~\ref{fig:chporefig2}, fine particle percolation behavior depends on the particle size ratio $R$ relative to $R_t$ resulting from bed particle size distribution half-width $w$. In the static bed consisting of size-monodisperse bed particles ($w=0$), for $R=6$, about 96.6\% fine particles are trapped after 1.5 s since $R<R_t$ (all fine particles will eventually be trapped, given longer simulation time). On the other hand, the fine particles continue percolating without being trapped for $R=7$. These two cases correspond exactly to the trapping and passing regimes observed in our previous work~\cite{gao2023percolation}. The fine particle spatial number distribution follows an approximately exponential relationship for the trapping regime and an approximately normal distribution for the passing regime (black curves), as previously explained~\cite{gao2023percolation}. 

When $w$ increases to 0.2, the theoretical trapping threshold becomes $R_t=8.080$, according to Eq.~\ref{eq:chporeeq1} for a triad of the smallest particles. However, fine particles with $R=8$ [right column of Fig.~\ref{fig:chporefig2}(b)] are seldomly trapped. Although the C1 condition describes the worst case, most bed particle triads in real packings form larger pore throats, such as the C2, C3, or C4 conditions. Nevertheless, a significant portion of fine particles, about 38.8\%, with $R=7$ are trapped within the simulation time of 1.5 s [see the left column of Fig.~\ref{fig:chporefig2}(b)], even though $R=7$ is well above $R_{t0}=6.464$ based on the average bed particle size. One should note that all fines with $R=7$ in this static bed will be trapped given sufficient simulation time. Figure~\ref{fig:chporefig2}(b) indicates that the theoretical pore-throat size based on the geometric perspective is only partially achieved in real packings. In other words, most pore throats are larger than the theoretical smallest bound. Moreover, in real random packings, the bed particle size distribution is more likely to be normal or log-normal rather than the uniform distribution used here, so the probability of the formation of the smallest pore throat becomes even less likely because most bed particles have diameters close to the average value. 

For $w=0.3$, where the effective free-sifting threshold becomes $R_t=9.234$, very few fine particles fines are trapped with $R=9$, but a small number of fines (about 18.8\%) with $R=8$ and a majority of fines (about 76.0\%) with $R=7$ are already trapped by the static bed within 1.5 s of simulation time. Again, given longer simulation time (although it depends on both $R$ and pore-throat size distribution~\cite{gao2023percolation}), all fines will be eventually trapped for $R=7$ and 8. It is important to note that even though the nominal free-sifting size ratio based on the average bed particle size occurs for $R>6.464$ (suggesting that no particles are trapped) in Figs.~\ref{fig:chporefig2}(b) and (c), when $w=0.2$ or $0.3$ significant numbers of fine particles are trapped even with $R>6.464$.


% which are commonly recognized as sufficiently large for free sifting since theirs values are obviously larger than the well-known number of $R_{t0}=6.464$.
%Although this further confirms that the theoretical limit obtained from the geometric perspective is not fully observed in reality, 


\subsection{Pore-throat size distribution for size-polydisperse static beds}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{ch_polyPSD_figures/Figure3.pdf}
    \caption{Pore-throat size distributions for static packings form by size-polydisperse bed particles with different particle size distribution half-width: (a) $w=0$, (b) $w=0.2$, and (c) $w=0.3$. The red vertical line denotes $d_p/d_0=1/6.464$, which is the lower bound given by the monodisperse packing limit. }
    \label{fig:chporefig3}
\end{figure}

To quantitatively show the effects of bed particle size variation on the pore-throat size distribution, we conduct Delaunay triangulation and further analysis to characterize the pore throats including their sizes and positions using the approaches described in the previous chapter~\cite{gao2023percolation}. Figure~\ref{fig:chporefig3}(a) demonstrates the pore-throat size distribution of the static bed formed by identical bed particles ($w=0$). Since all bed particles are identical, the densest arrangement of a planar triangle of three touching particles occurs frequently, corresponding to the data point at $d_p/d_0=1/6.464$ on the red vertical line. This gives rise to the high probability of the lower bound of $R_t=6.464$. However, the pore-throat size distribution extends below $d_p/d_0<1/6.464$ for $w=0.2$ and $w=0.3$, as shown in Figs.~\ref{fig:chporefig3}(b) and (c). This explains the phenomena observed in Figs.~\ref{fig:chporefig2}(b) and (c), where a significant portion of fines with $R=7$ and  8 are trapped by the static beds with bed particles having a range of sizes.


%It can be seen that barely no pore throat has the diameter less than $d/8$, while only a small fraction of them have the diameter less than $d/7$. This explains the phenomena observed in Fig.~\ref{fig:chporefig2}(b) that fines with $R=8$ are not trapped and only a small portion of fines with $R=7$ are trapped by the static bed. However, the theoretical free-sifting threshold for this case ($w=0.2$) is 8.080.  Similar phenomenon occurs for $w=0.3$ as well, see Fig.~\ref{fig:chporefig3}(c). 

%By obtaining the pore-throat size distribution, it is clear that increasing the bed particle distribution width can reduce the size of the narrowest constriction formed by the static bed, but not significantly as suggested by the theoretical value.
 
\section{Conclusion}

In this study, we focus on analyzing the void spaces, particularly pore throat sizes, within a static bed composed of size-polydisperse bed particles with varying size distribution widths. Through a purely geometric analysis, it is evident that an increase in the bed particle size distribution width results in the formation of smaller pore throats compared to the static beds formed by identical bed particles. 

%Moreover, we determine the theoretical free-sifting threshold as a function of the bed particle size distribution width theoretically. of fine particle percolation in static beds show that achieving the theoretical threshold in real packings occurs but is not dominant for $R$ near $R_{t0}=6.464$ because the theoretical limit is only reached when a planar triangle is formed by the three smallest bed particles tangent to one another. The limited number of smallest bed particles makes this configuration unlikely to occur frequently. Nevertheless, 

DEM simulations shows that even with a modest 20 to 30\% bed particle distribution half-width, a static bed can effectively trap a significant fraction of fine particles with a particle size ratio of $R=7$, specifically increasing from 0\% for $w=0$ (monodisperse packing) to 38.8\% for $w=0.2$ and 76.0\% for $w=0.3$ given a finite simulation time of 1.5 s. The fraction of trapped fine particles is further increased to 98.8\% as the bed particle distribution half-width reaches 0.5. $R=7$ is generally considered large enough to be sufficient for free sifting, but the smallest bed particles present in the broad particle size distribution create smaller pore throats that trap the fine particles. Therefore, it is crucial to understand how free sifting may be limited in practical industrial applications when there is a distribution of bed particle sizes. For instance, when designing granular beds for filtration purposes, the particle size distribution of the bed should be carefully considered to ensure the effective capture of impurities within the desired size range.



